More Church-Rosser Proofs in BELUGA

We report on yet another formalization of the Church-Rosser property in lambda-calculi, carried out with the proof environment Beluga. After the well-known proofs of confluence for beta-reduction in the untyped settings, with and without Takahashi's complete developments method, we concentrate on eta-reduction and obtain the result for beta-eta modularly. We further extend the analysis to typed-calculi, in particular System F. Finally, we investigate the idea of pursuing the encoding directly in Beluga's meta-logic, as well as the use of Beluga's logic programming engine to search for counterexamples.

==> eptcsdata.tex <==
\providecommand{\firstpage}{34}
\providecommand{\publicationstatus}{Temur Kutsia, Daniel Ventura, David Monniaux \&\\
 Jos\'e F. Morales (Eds.): LSFA 2023 + HCVS 2023\\
EPTCS 402, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.402.6}{10.4204/EPTCS.402.6}}

